Multi-Facet Recommender Networks with Spherical Optimization

Implicit feedback is widely explored by modern recommender systems. Since the feedback is often sparse and imbalanced, it poses great challenges to the learning of complex interactions among users and items. Metric learning has been proposed to capture user-item interactions from implicit feedback, but existing methods only represent users and items in a single metric space, ignoring the fact that users can have multiple preferences and items can have multiple properties, which leads to potential conflicts limiting their performance in recommendation. To capture the multiple facets of user preferences and item properties while resolving their potential conflicts, we propose the novel framework of Multi-fAcet Recommender networks with Spherical optimization (MARS). By designing a cross-facet similarity measurement, we project users and items into multiple metric spaces for fine-grained representation learning, and compare them only in the proper spaces. Furthermore, we devise a spherical optimization strategy to enhance the effectiveness and robustness of the multi-facet recommendation framework. Extensive experiments on six real-world benchmark datasets show drastic performance gains brought by MARS, which constantly achieves up to 40\% improvements over the state-of-the-art baselines regarding both HR and nDCG metrics.

==> comments_KDD.tex <==
Review 1

Suitability of paper to the Research Track
Relevance to KDD Research track:	
2: (Very relevant: the paper is interesting to most researchers in the area)
Double-blind review policy:	
0: (No)
No
Evaluation on the novelty, technical quality, impact, presentation, and reproducibility
Originality/Novelty:	
2: (Minor improvements over existing solutions)
Please justify your score for Originality/Novelty:	The paper proposes a MML model which can be regraded as an extension of Collaborative Metric Learning. The basic form of the proposed method in this paper is from CML, but authors incrementally improve it by adding treatments like "Adoption", "Exposure" and a calibrated sampling method.
Technical Quality:	
4: (Good technical work, properly evaluated)
Please justify your score for Technical Quality:	Experiments are well conducted. The authors also provide ablation study on the add-ons.
Impact/Outreach:	
3: (Fair solution to an important problem, but there are alternatives around)
Please justify your score for Impact/Outreach:	The problem in this paper is well-defined and widely studied. Various kinds of techniques and methods have been proposed in recent years to solve the implicit multi-facet recommendation problems. There is no obvious reason has been pointed out in the paper to justify why CML is a better choice than other alternatives.
Clarity of Presentation:	
4: (Paper is understandable but minor changes would make it accessible to a broader audience)
Reproducibility:	
4: (Yes - Good. It provides reasonably complete information that will help reproduce the results.)
Please justify your answer regarding Reproducibility:	The codes of CML based method is publicly available, and the add-ons proposed in this paper have been described well , and necessary parameters have been studied and evaluated.

Overall Evaluation

Three positive aspects of the paper:	

1. The paper follows the KDD paper fashion in terms of writing, presentation, and experiments. It is well-written, clear, and easy to follow.

2. The personalisation of margins for metric learning in this kind of problem settings seems interesting.

3. Experiments are well-conducted to showcase the superiority of the proposed MML method. Ablation study has been conducted as well to align the results to the claims of the paper.

Three negative aspects of the paper:	

1. The proposed MML model is incremental. MML builds upon CML model that was proposed in WWW 2017, and proposed several add-on treatments over the CML method, including "Adoption", "Exposure", as well as the "calibrated sampling method". That is to say, the novelty of this paper is limited and only includes the add-ons. In addition, Multiple space modelling is not new as well.

2. The presentation of this paper is not very well organised. For example, in section 3.1, the problem definition is incomplete, and the following section 3.2 "Challenges and motivation" is weird when placing it there. Personally, I would suggest to move it into introduction so that it can follow the logic of the paper.

3. There is no evaluation of scalability and efficiency of the proposed method. It is not clear how does MML perform when handling the large-scale datasets.

Overall Review:	See above positive and negative aspects.
Overall Evaluation:	
-2: (A below-the-bar paper (reject). I believe the paper is clearly below the standards for KDD.)
Overall Score:	
-2: (Reject)

-------------------------------------------------------------------------

Review 2
Suitability of paper to the Research Track
Relevance to KDD Research track:	
2: (Very relevant: the paper is interesting to most researchers in the area)
Double-blind review policy:	
0: (No)
no
Evaluation on the novelty, technical quality, impact, presentation, and reproducibility
Originality/Novelty:	
4: (Novel approach, using mature components in a novel way)
Please justify your score for Originality/Novelty:	The paper proposed a novel embedding method for recommender system, based on a tailored similarity function which switches the spaces depending on a given user-item pair.
Technical Quality:	
4: (Good technical work, properly evaluated)
Please justify your score for Technical Quality:	The basic idea would be reasonable, and I didn't find any significant flaw.
Impact/Outreach:	
4: (A good solution to a rather narrowly defined problem for a small target group of users)
Please justify your score for Impact/Outreach:	Although technical novelty is not super-strong, I think that the proposed method can be effective for the general recommender system problem.
Clarity of Presentation:	
4: (Paper is understandable but minor changes would make it accessible to a broader audience)
Reproducibility:	
4: (Yes - Good. It provides reasonably complete information that will help reproduce the results.)
Please justify your answer regarding Reproducibility:	The experimental setting is shown in detail.

Overall Evaluation
Three positive aspects of the paper:

- The issue focused by the paper would be interesting.
- The paper is well-organized.
- The empirical performance is evaluated exhaustively.

Three negative aspects of the paper:	- Technical novelty is not outstandingly strong (or not clearly described compared with existing multi-space metric learing)
- Many hyper-parameters exit, and some of them are set heuristically.
- Theoretical property of the proposed embedding is unclear.
Overall Review:	The paper proposes a method which embeds users and items into multiple spaces based on the implicit feedback matrix. The proposed method defines the triplet based loss function defined by combining K different embedded spaces, which is claimed as providing a richer embedding compared with the usual single space embedding. The authors also provide sampling procedure of training triplets based on interaction frequency. Prediction performance is examined through several benchmark datasets.

I think the basic idea would be reasonable, and motivation is clearly illustrated in Figure 1. Overall, I think the paper would provide an effective method for the general recommender system problem. The paper is well-organized, but several mathematical descriptions are a bit sloppy.

One concern is the technical novelty. The superiority compared with existing multi-space metric learning should have been described and/or compared. In particular, quantitative/qualitative advantage compared with [18] the authors cited would have been worth mentioning in more detail, because it has a similar formulation and learns multiple-metric though the metric is not adaptively chosen unlike the proposed method.

Many hyper-parameters exist, a part of which is fixed heuristically, but appropriateness of these settings are not fully clarified. For example, lambda_pull, the dimension of the embedding, K in NMF, alpha in NMF (6), gamma_u, alpha in (9) can be seen as hyper-parameters. The heuristics such (7) and (8) are seemingly practical, but the rationale behind it is not fully clarified.

The sampling criterion (12) is based on frequency of users and items. This is seemingly reasonable, but not rigorously justified.

Sometimes, mathematical descriptions are a bit confusing as listed below:

- After (6), the authors wrote ``||\cdot|| represents the squared sum''. What does this mean? Is it ``square-root of the squared sum''?

- In eq (6), P and Q in the constraints should be bold?

- For p(k|o), which first appears in (2), what does 'o' represent (a pair of a user and an item?).

- '\alpha' is used in (6) and (9) with different meanings. One of them should be changed.

- In eq (9), it would be better to explicitly indicate that p(k|o) in s(u,v) changes for each different pair of u and v. When I first read, I misunderstood that the function 's' is fixed for all the pair, though the weight p(k|o) depends on the input pair.

- What is definition of u* and v* in (11).

- In (4), why Q^T_{v,k} has 'transpose'? It is confusing because it is a scalar.
Overall Evaluation:	
-1: (An OK paper, but likely not good enough for KDD (weak reject). I vote for rejecting it, although I would not be upset if it were accepted.)
Overall Score:	
-1: (Weak reject)

--------------------------------------------------------------------------

Review 3
Suitability of paper to the Research Track
Relevance to KDD Research track:	
1: (Somehow relevant: the paper is interesting to some researchers in the area)
Double-blind review policy:	
0: (No)
No issues I could notice.
Evaluation on the novelty, technical quality, impact, presentation, and reproducibility
Originality/Novelty:	
4: (Novel approach, using mature components in a novel way)
Please justify your score for Originality/Novelty:	Novelty of the metric leaning problem and how it could model better than competitors is a meaningful technical advancement that is well-supported by examples. However, there is a lack of comparison to baselines developed for other domains (e.g., the KDD 2018 paper "PME: Projected Metric Embedding on Heterogeneous Networks for Link Prediction")
Technical Quality:	
4: (Good technical work, properly evaluated)
Please justify your score for Technical Quality:	Experiments and ablation analysis effectively show reasonable performance gains in diverse settings, though could explain differences in performance more concretely.
Impact/Outreach:	
4: (A good solution to a rather narrowly defined problem for a small target group of users)
Please justify your score for Impact/Outreach:	Is a proposed improved solution to a valuable problem that is validated on multiple diverse recommendation problems.
Clarity of Presentation:	
4: (Paper is understandable but minor changes would make it accessible to a broader audience)
Reproducibility:	
3: (Yes - Fair. The information provided represents a fair effort to make it possible for readers to reproduce the results.)
Please justify your answer regarding Reproducibility:	There isn’t a codebase, but it does discuss the data collection and parameter settings in detail. I would appreciate some more detail of an actual codebase and/or seeds/validation strategy.

Overall Evaluation

Three positive aspects of the paper:	

- The comparison to relevant related work in recommendation is succinct, comprehensive, and easy-to-follow. There is good contrast to similar ideas in literature (e.g., CML, weakness of certain margins, and pushing versus pulling).

- Technical contribution is well-developed and supported by examples in terms of the improvement and the challenges of the representation. The benefit and novelty of each component is well-discussed.

- Experiment improvements are impressive compared to diverse baselines. Ablation analysis is solid.

Three negative aspects of the paper:	

- The experiments do not dig deeper into why the models are better beyond ``these numbers are better.'' Some deeper insights of differences in recommendations for certain sets of a user or against common method would be valuable for showing the benefit of the approach.

- There are some unexplained performance differences, such as far smaller gaps for movielens, but there aren’t conjectures on why this is case. This sort of insight is important for validating the idea and better understanding when it is applicable. The inconsistency of some of the secondary performance is also a bit odd in terms of why methods are better or similar.

- Presentation could be polished further: there are a few more typos, odd phrasings, and editing issues than I would prefer.
Overall Review:	I would lean towards reject: the technical contribution is marred by presentation issues and additional verification of why the method is improved using deeper analysis. I think the paper is missing an ingredient of a deeper study of differences between the model beyond some of the visualization plots and conjectures; most descriptions seems improvements seem to be ``we said it would do this therefore it has to be doing this.’’

Another more pressing issue is that the related work doesn't consider other notions of multi-facet learning in other domains, such as "Projected Metric Embedding on Heterogeneous Networks for Link Prediction" paper or applications of computer vision of simultaneously considering multiple camera views. These sort of approaches represent a similar notion of ``multi-facet'' analysis even in a different domain and therefore should be compared to verify the approach, such as why these approaches are not compatible with the problem or how the notion of the methods' novelty compares.

Some Smaller Comments/Typos:
``Moivelens’’
``constitude’’
``framework with the state-of-the-art baseline result…’’ better to specify what the baseline is or mark the section it can be read about in.
- The base-m component seems to be rather marginal compared to the other gaps, though it does show that a combination of M+C does contribute. Some more insight on why that is the case would be valuable. I am not sure how valuable statistical intervals are with the leave-one-out framework but they could be included.

Overall Evaluation:	
-1: (An OK paper, but likely not good enough for KDD (weak reject). I vote for rejecting it, although I would not be upset if it were accepted.)
Overall Score:	
-1: (Weak reject)

--------------------------------------------------------------------------

Review 4
Suitability of paper to the Research Track
Relevance to KDD Research track:	
1: (Somehow relevant: the paper is interesting to some researchers in the area)
Double-blind review policy:	
0: (No)
The paper does not violate the double-blind review policy
Evaluation on the novelty, technical quality, impact, presentation, and reproducibility
Originality/Novelty:	
3: (Incremental)
Please justify your score for Originality/Novelty:	The existing metric learning methods represent users and items in a single space, ignoring the fact that users can have
multiple preferences and items can have multiple aspects, which limits the performance of recommendation. To fully represent the
multiple facets of users and items, the authors propose a Multi-facet Metric Learning (MML) framework. By designing a cross-space similarity measurement, they project users and items into multiple spaces for fine-grained representation
Technical Quality:	
4: (Good technical work, properly evaluated)
Please justify your score for Technical Quality:	The solution is technically sound; The claims made by the authors are well-supported by their findings; The authors validate according to the demands of the target grou
Impact/Outreach:	
3: (Fair solution to an important problem, but there are alternatives around)
Please justify your score for Impact/Outreach:	There is true need for the proposed solution. The proposed method overcome the limitation of traditional metric learning. Comprehensive experimental results clearly demonstrate the superiority of MML in comparison with various state-of-the-art
methods for recommendation. The experimental results are convincing.
Clarity of Presentation:	
4: (Paper is understandable but minor changes would make it accessible to a broader audience)
Reproducibility:	
4: (Yes - Good. It provides reasonably complete information that will help reproduce the results.)
Please justify your answer regarding Reproducibility:	The algorithms and resources used in a paper were described to allow for reproducibility?

Overall Evaluation
Three positive aspects of the paper:	

1. The authors study the challenge of recommendation with implicit feedback and spot the inefficacy of existing methods in modeling
and optimizing towards multi-facet user preferences and item aspects. This is a meaningful problem.
2. The motivation of this paper of is clear
3. This paper is well-organized.

Three negative aspects of the paper:	

1. Some explanations are deficient. For example, what the differences between the proposed methods with multi-view metric learning methods?
2. The analysis of algorithm is not enough. For example. the convergence or complexity of the proposed algorithm is not provided
Overall Review:	The authors propose a Multi-facet Metric Learning (MML) framework for recommendation with implicit feedback. They firstly
use NMF to initialize multiple metric spaces without any auxiliary information and obtain the corresponding projection intensity of
users and items. Then they design a cross-space similarity measurement for users and items under a multi-space scenario. This method can effectively combine multiple facets of users and items for more fine-grained modeling. However, please address the above problems .

Overall Evaluation:	
1: (An OK paper, good enough for KDD (weak accept). Accept if possible, although I would not be upset if it were rejected.)
Overall Score:	
-1: (Weak reject)
